ProDMPs: A Unified Perspective on Dynamic and Probabilistic Movement Primitives

Movement Primitives (MPs) are a well-known concept to represent and generate modular trajectories. MPs can be broadly categorized into two types: (a) dynamics-based approaches that generate smooth trajectories from any initial state, e. g., Dynamic Movement Primitives (DMPs), and (b) probabilistic approaches that capture higher-order statistics of the motion, e. g., Probabilistic Movement Primitives (ProMPs). To date, however, there is no method that unifies both, i. e. that can generate smooth trajectories from an arbitrary initial state while capturing higher-order statistics. In this paper, we introduce a unified perspective of both approaches by solving the ODE underlying the DMPs. We convert expensive online numerical integration of DMPs into basis functions that can be computed offline. These basis functions can be used to represent trajectories or trajectory distributions similar to ProMPs while maintaining all the properties of dynamical systems. Since we inherit the properties of both methodologies, we call our proposed model Probabilistic Dynamic Movement Primitives (ProDMPs). Additionally, we embed ProDMPs in deep neural network architecture and propose a new cost function for efficient end-to-end learning of higher-order trajectory statistics. To this end, we leverage Bayesian Aggregation for non-linear iterative conditioning on sensory inputs. Our proposed model achieves smooth trajectory generation, goal-attractor convergence, correlation analysis, non-linear conditioning, and online re-planing in one framework.

==> figure/tex/agg_sample_one_image.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \begin{minipage}[t!]{\linewidth}
        \includegraphics[width=\linewidth]{figure/pdf/agg_one_img/agg_6_1.pdf}
        \label{fig:digit_replan2}
        \vspace{-4mm}
        % \subcaption[]{}
    \end{minipage}
    \begin{minipage}[t!]{\linewidth}
        \includegraphics[width=\linewidth]{figure/pdf/agg_one_img/agg_6_2.pdf}
        \label{fig:digit_replan3}
        \vspace{-4mm}
        % \subcaption[]{}
    \end{minipage}
    \begin{minipage}[t!]{\linewidth}
        \includegraphics[width=\linewidth]{figure/pdf/agg_one_img/agg_6_3.pdf}
        \label{fig:digit_replan_3_to_2}
        \vspace{-4mm}
        % \subcaption[]{}
    \end{minipage}
    \begin{minipage}[t!]{\linewidth}
        \includegraphics[width=\linewidth]{figure/pdf/agg_one_img/agg_8_1.pdf}
        \label{fig:digit_replan2}
        \vspace{-4mm}
        % \subcaption[]{}
    \end{minipage}
    \begin{minipage}[t!]{\linewidth}
        \includegraphics[width=\linewidth]{figure/pdf/agg_one_img/agg_8_2.pdf}
        \label{fig:digit_replan3}
        \vspace{-4mm}
        % \subcaption[]{}
    \end{minipage}
    \begin{minipage}[t!]{\linewidth}
        \includegraphics[width=\linewidth]{figure/pdf/agg_one_img/agg_8_3.pdf}
        \label{fig:digit_replan_3_to_2}
        \vspace{-4mm}
        % \subcaption[]{}
    \end{minipage}
    \caption{Prediction of digit writing trajectories conditioned on up to 3 noisy version of an image.}
    \label{fig:digit_agg_one_img}
\end{wrapfigure}




==> figure/tex/blending.tex <==
\begin{figure}[t!]
\vspace{-5mm}
\centering
\subcaptionbox{Demonstrations\label{fig:two_demo}}
[.32\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/blending/demo.pdf}
}%
\hfill
\subcaptionbox{Combination\label{fig:combination}}
[.32\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/blending/Combination.pdf}
}%
\hfill
\subcaptionbox{Blending\label{fig:blending}}
[.32\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/blending/Blending.pdf}
}%
\caption{We illustrate combination and blending two demonstrated trajectory distributions using \acrshortpl{pdmp}. The blue and red colors indicate two demonstrated trajectory distributions, and the green color indicates the resulting combination and blending trajectory distribution. The $\times$ shape markers are the via-points.}
\label{fig:prodmp_blending}
\vspace{-0.4cm}
\end{figure}


==> figure/tex/cov_learning.tex <==
\begin{figure}[t!]
% \vspace{-0.2cm}
% \begin{wrapfigure}{r}{0.55\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\centering
\subcaptionbox{\label{fig:optimal_control}}
[.29\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/cov_learning/oc_dataset.pdf}
}%
\hfill
\subcaptionbox{\label{fig:oc_promp_decouple}}
[.25\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/cov_learning/oc_promp_decouple.pdf}
}%
\hfill
\subcaptionbox{\label{fig:oc_promp}}
[.25\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/cov_learning/oc_promp.pdf}
}%
\vspace{-0.6cm}
\caption{Illustration of learning trajectory's temporal correlation using one or two time steps. We predict the prior trajectories distribution given no observation, and sample trajectories from it. To clearly demonstrate the difference, we do not use boundary condition terms. \textbf{Left}: Dataset generated by stochastic optimal control using one high-cost via-point at $t=50$ and one low-cost via-point at $t=80$. \textbf{Middle}: Maximizing the likelihood of one single time step's position cannot learn the temporal correlation properly. \textbf{Right}: Using two time steps jointly in Eq.(\ref{eq:rec_ll}) captures the temporal correlation correctly. }
\label{fig:temporal_cov}
\vspace{-0.5cm}
\end{figure}


==> figure/tex/digit_replan.tex <==
\begin{wrapfigure}{t}{0.5\textwidth}
    % \begin{minipage}[t!]{\linewidth}
    %     \includegraphics[width=\linewidth]{figure/pdf/digit_replan/digit_replan_2.pdf}
    %     \label{fig:digit_replan2}
    %     \vspace{-4mm}
    %     % \subcaption[]{}
    % \end{minipage}
    % \begin{minipage}[t!]{\linewidth}
    %     \includegraphics[width=\linewidth]{figure/pdf/digit_replan/digit_replan_3.pdf}
    %     \label{fig:digit_replan3}
    %     \vspace{-4mm}
    %     % \subcaption[]{}
    % \end{minipage}
    \begin{minipage}[t!]{\linewidth}
        \includegraphics[width=\linewidth]{figure/pdf/digit_replan/digit_replan_3to2.pdf}
        \label{fig:digit_replan_3_to_2}
        \vspace{-4mm}
        % \subcaption[]{}
    \end{minipage}
    \caption{Three-step online replanning in digit writing task.}
    \label{fig:digit_replan}
\end{wrapfigure}


==> figure/tex/dmp_vs_idmp.tex <==
\begin{wrapfigure}{r}{0.32\textwidth}
\vspace{-4.5mm}
    \centering
  \includegraphics[width=0.32\textwidth]{figure/pdf/pos1.pdf}
  \caption{The \acrshortpl{pdmp} and \acrshortpl{dmp} generate identical trajectory. However our method uses linear basis functions instead of online numerical integrals.}
  \label{fig:dmp_vs_idmp}
\vspace{-0.2cm}
\end{wrapfigure}

==> figure/tex/idmp_pos_vel.tex <==
\begin{figure*}[t!]
    \begin{center}
    \vspace{-0.5cm}
    \hspace{0.06cm}
    \subcaptionbox{Position (mean)\label{fig:idmp_pos}}[0.315\textwidth]{
        \includegraphics[width=0.305\textwidth]{figure/pdf/idmp_pos_vel/pos.pdf}
        \vspace{-0.1cm}}
    \hfill
    \subcaptionbox{Position std \label{fig:idmp_pos_std}}[0.32\textwidth]{
        \includegraphics[width=0.31\textwidth]{figure/pdf/idmp_pos_vel/pos_std.pdf}
        \vspace{-0.1cm}}
    \hfill
    \subcaptionbox{Position samples \label{fig:idmp_pos_smp}}[0.32\textwidth]{
        \includegraphics[width=0.31\textwidth]{figure/pdf/idmp_pos_vel/smp.pdf}
        \vspace{-0.1cm}}
    \hfill
    \subcaptionbox{Velocity (mean) \label{fig:idmp_vel}}[0.325\textwidth]{
        \includegraphics[width=0.313\textwidth]{figure/pdf/idmp_pos_vel/vel.pdf}
        \vspace{-0.1cm}}
    \hfill
    \subcaptionbox{Velocity std \label{fig:idmp_vel_std}}[0.32\textwidth]{
        \includegraphics[width=0.31\textwidth]{figure/pdf/idmp_pos_vel/vel_std.pdf}
        \vspace{-0.1cm}}
    \hfill
    \subcaptionbox{Velocity samples \label{fig:idmp_vel_smp}}[0.32\textwidth]{
        \includegraphics[width=0.31\textwidth]{figure/pdf/idmp_pos_vel/vel_smp.pdf}
        \vspace{-0.1cm}}
  \end{center}
  \vspace{-0.2cm}
  \caption{Trajectory position and velocity of \acrshortpl{pdmp}. x-axis: time, y-axis: position or velocity. Our model can generate not only the (a) position and (d) velocity of the original \acrshortpl{dmp} framework, but also their variance in (b)(e) respectively. Similar to \acrshortpl{promp}, \acrshortpl{pdmp} can also be used as a generative model to get trajectory samples. Here, all sampled trajectories follow the same boundary condition, i.e. $\text{position}=5$, $\text{velocity}=-5$.}
  \label{fig:idmp_pos_vel}
\end{figure*}

==> figure/tex/idmp_vel_basis.tex <==
% \begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}[t!]
% \vspace{-3.5mm}
  \begin{center}
    \subcaptionbox{Weights' basis \label{fig:idmp_basis_pw}}[0.243\textwidth]{
      \includegraphics[width=\linewidth]{figure/pdf/v_basis_w.pdf}\vspace{-0.15cm}}
      \hfill
    \subcaptionbox{Goal's basis \label{fig:idmp_basis_pg}}[0.23\textwidth]{
  \includegraphics[width=\linewidth]{figure/pdf/v_basis_g.pdf}\vspace{-0.15cm}}
  \end{center}
  \vspace{-0.25cm}
  \caption{The velocity basis functions of the \acrshort{pdmp}s, corresponding to the position basis functions in Fig. \ref{fig:idmp_basis}.}
  \label{fig:idmp_vel_basis}
% \vspace{-4mm}
\end{figure}
% \end{wrapfigure}


==> figure/tex/noisy_digit_additional.tex <==
\begin{figure}[h]
\captionbox{More sampled trajectories, from prediction given three noisy images.\label{fig:noisy_digit_supplementary}\vspace{-0.2cm}}
[\textwidth]{
    % \subcaptionbox{}
    % [.48\textwidth]{
    %     \includegraphics[width=\linewidth]{figure/pdf/noisy_digit_additional/noisy_additional1.pdf}
    % }%
    % \subcaptionbox{}
    % [.48\textwidth]{
    %     \includegraphics[width=\linewidth]{figure/pdf/noisy_digit_additional/noisy_additional2.pdf}
    % }%
    \includegraphics[width=0.8\linewidth]{figure/pdf/noisy_digit_additional/3.pdf}  
    }
    \vspace{-2cm}
\end{figure}

==> figure/tex/robot_pick_additional.tex <==
\begin{figure}[h]
\vspace{0.1cm}
\captionsetup[subfigure]{labelformat=empty}
\centering
\begin{minipage}[b]{0.1\textwidth}
    step 1 \\
    
    \vspace{0.12cm}
    
    step 2 \\
    
    \vspace{0.12cm}
    
    step 3 \\
    
    \vspace{0.12cm}
    
    step 4 \\
    
    \vspace{0.12cm}
\end{minipage}
\subcaptionbox{\acrshort{dof} 1}
[.22\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/robot_pick/var_0.pdf}
}%
\hfill
\subcaptionbox{\acrshort{dof} 2}
[.22\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/robot_pick/var_1.pdf}
}%
\hfill
\subcaptionbox{\acrshort{dof} 3}
[.22\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/robot_pick/var_2.pdf}
}%
\hfill
\subcaptionbox{\acrshort{dof} 4}
[.22\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/robot_pick/var_3.pdf}
}%
\vspace{0.2cm}
\hfill
\begin{minipage}[b]{0.1\textwidth}
    step 1 \\
    
    \vspace{0.12cm}
    
    step 2 \\
    
    \vspace{0.12cm}
    
    step 3 \\
    
    \vspace{0.12cm}
    
    step 4 \\
    
    \vspace{0.12cm}
\end{minipage}
\subcaptionbox{\acrshort{dof} 5}
[.22\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/robot_pick/sam_4.pdf}
}%
\subcaptionbox{\acrshort{dof} 6}
[.22\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/robot_pick/sam_5.pdf}
}%
\subcaptionbox{\acrshort{dof} 7}
[.22\textwidth]{
    \includegraphics[width=\linewidth]{figure/pdf/robot_pick/sam_6.pdf}
}%
\hfill
\caption{Supplementary joint trajectories plots in 4-step replanning of the robot picking task. Here, we plot the mean and variance of the first 4 \acrshortpl{dof}, while plotting the mean and samples of the last 3 \acrshortpl{dof}. The dark gray dashed lines are human's demonstrations. The variance of the trajectory decreases drastically after the object shifted its position.}
\label{fig:robot_pick_additional}
\vspace{-0.3cm}
\end{figure}


==> figure/tex/robot_pick_demo_vs_predict.tex <==
\begin{wrapfigure}{r}{0.35\textwidth}
\vspace{-20.5mm}
    \centering
  \includegraphics[width=0.35\textwidth]{figure/pdf/robot_pick/demo_vs_predict.png}
  \caption{\acrshortpl{pdmp} learn fast correction motion from human demonstration. In current example, the object to be picked up has shifted 40 cm.}
  \label{fig:robot_pick_demo_vs_predict}
\vspace{-0.2cm}
\end{wrapfigure}

==> figure/tex/robot_push_illustration.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \vspace{-0.5cm}
    \includegraphics[width=\linewidth]{figure/screenshot/illustration.png}
\caption{Illustration of pushing and replanning task. \label{fig:robot_push_illustration}}
\end{wrapfigure}



==> table/List_of_symbols.tex <==
\renewcommand{\arraystretch}{1.33}
% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
\begin{table}[htbp]
    \small
    \centering
    % \vspace{-0.7cm}
    \caption{List of symbols used in this paper.\vspace{0.2cm}}
    \begin{tabular}{cm{12.8cm}}
        \toprule
        \textbf{Symbol} & \textbf{Description}\\
        \hline
        $ b $ & The time step of the boundary conditions \\
        $ c $ & Coefficients of the general solutions of \acrshortpl{dmp}' \acrshort{ode} \\
        $ d,~D $ & Index and the number of \acrshortpl{dof} \\
        $ f $ & Forcing function of the original \acrshortpl{dmp} \\
        $ F $ & The source term in the \acrshortpl{dmp}'non-homogeneous \acrshortpl{ode} \\
        $ g $ & The Goal term of \acrshortpl{dmp} and \acrshortpl{pdmp}\\
        % $ h $ &  \\
        $ \bm{H} $ & A combination of \acrshortpl{pdmp}' basis and boundary conditions terms, used in distribution computation \\
        $ i $ & Index of the basis functions and weights of one \acrshort{dof}\\
        $ j,~J $ & Index and the total number of the randomly selected time pairs used in loss computation \\
        $ k $ & Index of the boundary condition terms \\
        $ I $ & The two indefinite integrals in the closed form solution of \acrshortpl{dmp}' \acrshort{ode} \\
        $ \bm{L} $ & The Cholesky decomposition of a covariance matrix \\
        $ \mathcal{L} $ & The loss function to be minimized \\
        $ N $ & The number of basis functions and weights per \acrshortpl{dof}  \\
        $ m,~M $ & Index and the number of observations \\
        $ \bm{o},~\mathcal{O} $ & Sensory observation and a set of observations \\
        $ \bm{p} $ & The first definite integral in $I$ which must be computed using a numerical integral \\
        $ q $ & The second definite integral in $I$ which can be solved analytically\\
        $ \bm{r} $ & Latent observation \\
        $ t, T $ & Index of time steps and the length of trajectory, i.e. the number of total time steps \\
        $ \bm{w}, \bm{w_g} $ & The weights of \acrshortpl{dmp}, \acrshortpl{promp}, and \acrshortpl{pdmp}. A concatenation of weights and goal.\\
        $ x $ & The phase of the canonical system, which decays exponentially w.r.t time. \\
        $ y, ~\dot{y},~ \ddot{y} $ & One \acrshort{dof} trajectory position, velocity, and acceleration of a single time step respectively \\
        $ \bm{y} $ & $D$-\acrshortpl{dof} trajectory position of a single time step \\
        $ Y $ & The denominator in the indefinite integrals $I_1$ and $I_2$\\
        $ \bm{z} $ & The latent variable in Neural Processes, Bayesian Aggregation and \acrshortpl{pdmp}' deep embeddings \\
        \midrule
        $ \alpha_x $ & Exponential decaying coefficient of the canonical system \\
        $ \alpha, \beta $ & Spring-damper coefficient of \acrshortpl{dmp}  \\
        $ \Delta  $ & The characteristic equation of \acrshortpl{dmp}' homogeneous \acrshortpl{ode}\\
        $ \epsilon $ & Gaussian white noise \\
        $ \theta $ & Neural Networks' learnable parameters \\
        $ \bm{\lambda}, \bm{\Lambda} $ & A single \acrshort{dof} trajectory and a multi \acrshortpl{dof} trajectory \\
        $ \mu, \bm{\mu} $ & The mean of a certain probabilistic distribution \\
        $ \xi,~\bm{\xi} $ & One or multi time-step term determined by boundary conditions in \acrshortpl{pdmp}' trajectory computation \\
        % $ \pi $ &  \\
        $ \sigma^2 $ & The variance of a certain probabilistic distribution \\
        $ \bm{\Sigma} $ & The covariance of a certain probabilistic distribution \\
        $ \tau $ & Time scaling factor of \acrshortpl{dmp}, determining the execution speed \\
        $ \bm{\varphi} $ & Basis function forming up \acrshortpl{dmp}' forcing term \\
        $ \bm{\Phi} $ & Basis functions of one \acrshort{dof} used by \acrshortpl{promp} and \acrshortpl{pdmp}, written in matrix \\
        $ \bm{\Psi} $ & Blocked diagonal basis function matrix used by \acrshortpl{promp} and \acrshortpl{pdmp} for multi \acrshortpl{dof} trajectory \\
        $ \dot{\bm{\Phi}}, \dot{\bm{\Psi}} $ & Single and blocked diagonal velocity basis function matrices \\
        % $  $ &  \\
        \bottomrule
    \end{tabular}
     \vspace{-.5cm}
    \label{tab:model_comparison}
\end{table}
\renewcommand{\arraystretch}{1}

==> table/Speedtest.tex <==
\renewcommand{\arraystretch}{1.5}
\captionsetup[table]{position=top}
\begin{table}[htbp]
    \vspace{-0.4cm}
    % \footnotesize
    \scriptsize
    \centering
    \caption{Speed comparison of forward and backward pass between NN-\acrshortpl{dmp} and \acrshortpl{pdmp}. Our model is 200-4600 times faster in different settings. Here the trajectory has 6-second length, 1000 Hz frequency, 2-\acrshortpl{dof}, and 22-dim for $\bm{w}_g$. The result is achieved by a Nvidia\textregistered ~GeForce\textregistered ~RTX-3080Ti GPU. \label{tab: speed_test}}

    \subcaptionbox[position=top]{Forward pass \label{tab:fast_and_furious}}
    {
        \begin{tabular}{ccc}
        \toprule
        \textbf{Pipelines} & \centering \textbf{NN-based \acrshortpl{dmp}} & \textbf{\acrshortpl{pdmp}} \\
        \hline
        Renew BC & $\ccm$  & $\ccm$ \\
        Avg. time & 0.6145 s  & 0.0027 s \\
        \textbf{Relative speed} & 1  & \textbf{227.59} \\
        \hline
        Renew BC & $\times$  & $\times$ \\
        Avg. time & 0.6057 s  & 0.00013 s \\
        \textbf{Relative speed} & 1  & \textbf{4653.84} \\
        \hline
        \bottomrule
        \end{tabular}
    }
    \hspace{0.2cm}
    % \hfill
    \subcaptionbox[position=top]{Back-propagation \label{tab:fast_and_furious_back}}{
        \begin{tabular}{ccc}
        \toprule
        \textbf{Pipelines} & \centering \textbf{NN-based \acrshortpl{dmp}} & \textbf{\acrshortpl{pdmp}} \\
        \hline
        Renew BC & $\ccm$  & $\ccm$ \\
        Avg. time & 1.5737 s  & 0.0039 s \\
        \textbf{Relative speed} & 1  & \textbf{403.51} \\
        \hline
        Renew BC & $\times$  & $\times$ \\
        Avg. time & 1.5261 s  & 0.00105 s \\
        \textbf{Relative speed} & 1  & \textbf{1453.42} \\
        \hline
        \bottomrule
    \end{tabular}
    }
% \vspace{0.8cm}
\end{table}


==> table/input_output.tex <==
\renewcommand{\arraystretch}{1.5}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{table}[t]
    \scriptsize
    \centering
    \vspace{0.1cm}
    \caption{Dimensions of the variables in Eq.(\ref{eq:idmp_mean_cov}), where dim\_$\bm{w}_g =$ dim\_dof $\times$ num\_basis\_per\_dof. We use $\times$ to denote a coupling of two dimensions into one dimension, and "," to distinguish different dimensions of the variable.}
    \begin{tabular}{cc}
        \toprule
        \textbf{Variable} & \textbf{Dimension} \rule{0pt}{3.5mm}\\
        \hline
        $\bm{w}_g,~\bm{\mu}_{\bm{w}_g}$ & [dim\_$\bm{w}_g$]\\ $\bm{\Sigma}_{\bm{w}_g}$& [dim\_$\bm{w}_g$, dim\_$\bm{w}_g$]\\ $\bm{y}_b, ~\dot{\bm{y}}_b$ & [num\_dof]\\
        $\bm{\Lambda},~\bm{\mu}_{\Lambda}$ & [num\_dof $\times$ num\_times] \\ $\bm{\Sigma}_{\Lambda}$ &  [num\_dof $\times$ num\_times, num\_dof $\times$ num\_times] \\ $\bm{\xi}_k$ & [num\_times] \\
        $\bipbb,~\bivbb$ & [dim\_$\bm{w}_g$, num\_dof] \\ $\bipb_{0:T},~ \bm{H}_{0:T}$ & [dim\_$\bm{w}_g$, num\_dof $\times$ num\_times] \\
        \bottomrule
    \end{tabular}
    \label{tab:dim_variables}
    % \vspace{-1cm}
\end{table}
\renewcommand{\arraystretch}{1}

==> table/model_compare.tex <==
\newcommand{\ccm}{\hfil \checkmark}
\renewcommand{\arraystretch}{1.3}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\setcounter{table}{3}
% \captionsetup{font=footnotesize}
% \begin{wrapfigure}{r}{0.63\textwidth}
\begin{table}[t!]
    \centering
        \scriptsize
        \centering
        % \vspace{-4.5mm}
        \captionof{table}{A comparison between our \acrshortpl{pdmp} and previous models. The NN-\acrshortpl{dmp} method is using a probabilistic approach only in the RL case \cite{bahl2020neural} for the weights, and can thus not directly model trajectory distributions. We marked its entry as '$\sim$'.\label{tab:model_comparison}}
        \begin{tabular}{m{2cm}cccc>{\columncolor[HTML]{EAEDED}}c}
            \toprule
            \textbf{Features} & \centering \textbf{\acrshort{dmp}} & \centering \textbf{\acrshort{promp}} & \centering \textbf{\acrshort{cnmp}}
            & \centering \textbf{NN-\acrshort{dmp}} &  \textbf{\acrshort{pdmp}} \rule{0pt}{3.3mm}\\
            \hline
            Model dynamics & \ccm & \centering $\times$ & \centering $\times$ & \ccm & \ccm\\
            % \hline
            Model statistics & \centering $\times$  & \ccm & \ccm & \centering \centering $\sim$ &\ccm\\
            % \hline
            Model covariance & \centering $\times$  & \ccm & \centering $\times$   & \centering $\times$  & \ccm\\
            % \hline
            High-dim. input & \centering $\times$  & \centering $\times$  & \ccm & \ccm & \ccm\\
            % \hline
            Partial observation & \centering $\times$ &  \centering $\times$ &  \centering $\times$  &  \centering $\times$ & \ccm\\
            % \hline 
            No online integral & \centering $\times$ &  \ccm &  \ccm  &  \centering $\times$ & \ccm\\
            \bottomrule
        \end{tabular}
%  \vspace{-0.4cm}
\end{table}
% \end{wrapfigure}


==> table/smoothness.tex <==
\begin{wraptable}{l}{0.6\textwidth}
\renewcommand{\arraystretch}{1.5}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
% \begin{table}[htbp]
    \scriptsize
    \centering
    \vspace{-0.5cm}
    \caption{Trajectory smoothness measure in box pushing task.}
    \begin{tabular}{c|ccc}
        \toprule
        &\acrshortpl{pdmp} &\acrshortpl{pdmp}(std)& CNMP \\
        \hline
        Average Squared Acceleration& 3.31 & 4.65 & 800.54  \\
        Log Dimensionless Jerk (LDLJ)\cite{balasubramanian2015analysis} &-20.15 & -20.22 & -23.80 \\
        \bottomrule
    \end{tabular}
    \vspace{0.2cm}
    \label{tab:smoothness}
    % \vspace{-0.2cm}
% \end{table}
\renewcommand{\arraystretch}{1}
\end{wraptable}
